The Role of Verb Semantics in Hungarian Verb-Object Order

Hungarian is often referred to as a discourse-configurational language, since the structural position of constituents is determined by their logical function (topic or comment) rather than their grammatical function (e.g., subject or object). We build on work by Koml\'osy (1989) and argue that in addition to discourse context, the lexical semantics of the verb also plays a significant role in determining Hungarian word order. In order to investigate the role of lexical semantics in determining Hungarian word order, we conduct a large-scale, data-driven analysis on the ordering of 380 transitive verbs and their objects, as observed in hundreds of thousands of examples extracted from the Hungarian Gigaword Corpus. We test the effect of lexical semantics on the ordering of verbs and their objects by grouping verbs into 11 semantic classes. In addition to the semantic class of the verb, we also include two control features related to information structure, object definiteness and object NP weight, chosen to allow a comparison of their effect size to that of verb semantics. Our results suggest that all three features have a significant effect on verb-object ordering in Hungarian and among these features, the semantic class of the verb has the largest effect. Specifically, we find that stative verbs, such as fed "cover", jelent "mean" and \"ovez "surround", tend to be OV-preferring (with the exception of psych verbs which are strongly VO-preferring) and non-stative verbs, such as b\'ir\'al "judge", cs\"okkent "reduce" and cs\'okol "kiss", verbs tend to be VO-preferring. These findings support our hypothesis that lexical semantic factors influence word order in Hungarian.

==> wont_add/information_theoretic_exp.tex <==
\section{An Information Theoretic Model}

\subsection{Methods}

\todo{write section}
\paragraph{Logistic Regression.}

\paragraph{Pointwise Mutual Information.}

\paragraph{Conditional Probabilities.}

\paragraph{Multicollinearity.} PMI is highly correlated with both $p(o|v)$ and $p(v|o)$. Hence, we residualize PMI against $p(o|v)$ and $p(v|o)$.

\subsection{Results}

We find that $p(v|o)$ explains most of the variance. 

These factors have different effects on different verbs.  significant effect of $p(v|o)$

==> wont_add/verb_table.tex <==
\begin{longtable}{|lllccccc|}
\hline 
\hline
\textbf{ID} & \textbf{Verb Lemma}                                                                  & \textbf{Translation}                                                                                                                 & \textbf{Pref.} & \textbf{Log Odds} & \textbf{$z$-score} & \textbf{Category}    & \textbf{Freq.}                                               \\ \hline
\endfirsthead
%
\endhead
%
1	 &	aggaszt	 &	worry	 &	OV	 &	-0.81	 &	-7.85	 &	\textsc{change}	 &	444	\\ \hline
2	 &	\begin{tabular}[c]{@{}l@{}}akadályoz/\\ akadályozik\end{tabular}	 &	obstruct	 &	VO	 &	0.89	 &	8.08	 &	\textsc{affect}	 &	3031	\\ \hline
3	 &	aktivál	 &	activate	 &	VO	 &	0.76	 &	5.41	 &	\textsc{change}	 &	488	\\ \hline
4	 &	aktivizál	 &	\begin{tabular}[c]{@{}l@{}}get someone to\\ take action\end{tabular}	 &	VO	 &	1.32	 &	4.98	 &	\textsc{change}	 &	100	\\ \hline
5	 &	alkalmaz	 &	\begin{tabular}[c]{@{}l@{}}employ,\\ implement\end{tabular}	 &	OV	 &	-1.6	 &	-11.74	 &	\textsc{activity}	 &	888	\\ \hline
6	 &	alkot	 &	create, form	 &	OV	 &	-1.08	 &	-10.24	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	9081	\\ \hline
7	 &	áramtalanít	 &	de-electrify	 &	no sig.	 &	0.4	 &	1.89	 &	\textsc{change}	 &	122	\\ \hline
8	 &	árnyal	 &	\begin{tabular}[c]{@{}l@{}}make nuanced,\\ complicate\end{tabular}	 &	VO	 &	0.54	 &	3.61	 &	\textsc{change}	 &	369	\\ \hline
9	 &	\begin{tabular}[c]{@{}l@{}}bántalmaz/\\ bántalmazik\end{tabular}	 &	hurt, abuse	 &	VO	 &	0.52	 &	4.34	 &	\textsc{affect}	 &	1165	\\ \hline
10	 &	befolyásol	 &	influence	 &	VO	 &	0.46	 &	4.39	 &	\textsc{affect}	 &	9720	\\ \hline
11	 &	bírál	 &	judge, evaluate	 &	VO	 &	0.95	 &	8.71	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	3879	\\ \hline
12	 &	birtokol	 &	own, possess	 &	OV	 &	-0.53	 &	-4.51	 &	\textsc{ownership}	 &	1309	\\ \hline
13	 &	blokkol	 &	block	 &	VO	 &	0.71	 &	4.88	 &	\textsc{affect}	 &	417	\\ \hline
14	 &	bojkottál	 &	boycott	 &	VO	 &	1.08	 &	7.53	 &	\textsc{affect}	 &	525	\\ \hline
15	 &	boncolgat	 &	\begin{tabular}[c]{@{}l@{}}anatomize\\ (iterative)\end{tabular}	 &	OV	 &	-1.66	 &	-8.02	 &	\textsc{change}	 &	231	\\ \hline
16	 &	bontogat	 &	unfold (iterative)	 &	VO	 &	0.57	 &	2.59	 &	\textsc{change}	 &	116	\\ \hline
17	 &	bonyolít	 &	complicate	 &	OV	 &	-0.26	 &	-2.16	 &	\textsc{change}	 &	1090	\\ \hline
18	 &	borít	 &	cover	 &	OV	 &	-1.21	 &	-10.68	 &	\textsc{covering}	 &	2486	\\ \hline
19	 &	cáfol	 &	refute	 &	VO	 &	1.32	 &	11.69	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	2643	\\ \hline
20	 &	\begin{tabular}[c]{@{}l@{}}céloz/\\ célozik\end{tabular}	 &	aim at	 &	OV	 &	-3.57	 &	-18.76	 &	\textsc{preference}	 &	1465	\\ \hline
21	 &	\begin{tabular}[c]{@{}l@{}}cenzúráz/\\ cenzúrázik\end{tabular}	 &	censor	 &	no sig.	 &	0.13	 &	0.61	 &	\textsc{affect}	 &	128	\\ \hline
22	 &	csapkod	 &	hit at	 &	VO	 &	0.47	 &	2.87	 &	\textsc{affect}	 &	260	\\ \hline
23	 &	cserélget	 &	switch, replace	 &	VO	 &	1.29	 &	5.51	 &	\textsc{change}	 &	134	\\ \hline
24	 &	csillapít	 &	soothe	 &	VO	 &	0.65	 &	4.53	 &	\textsc{change}	 &	438	\\ \hline
25	 &	csodál	 &	admire	 &	VO	 &	0.89	 &	6.67	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	676	\\ \hline
26	 &	csökkent	 &	reduce	 &	VO	 &	1.3	 &	12.29	 &	\textsc{change}	 &	8782	\\ \hline
27	 &	csókol	 &	kiss	 &	OV	 &	-1.22	 &	-9.59	 &	\textsc{affect}	 &	1013	\\ \hline
28	 &	csókolgat	 &	kiss	 &	no sig.	 &	-0.03	 &	-0.14	 &	\textsc{affect}	 &	144	\\ \hline
29	 &	csorbít	 &	impair	 &	VO	 &	0.47	 &	3.11	 &	\textsc{change}	 &	353	\\ \hline
30	 &	csóvál	 &	frisk	 &	VO	 &	0.36	 &	2.92	 &	\textsc{affect}	 &	855	\\ \hline
31	 &	dédelget	 &	fondle, pamper	 &	OV	 &	-0.94	 &	-4.74	 &	?	 &	174	\\ \hline
32	 &	dicsér	 &	praise	 &	no sig.	 &	0.04	 &	0.37	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	2163	\\ \hline
33	 &	dicsőít	 &	glorify	 &	no sig.	 &	0.25	 &	1.5	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	231	\\ \hline
34	 &	diktál	 &	dictate	 &	no sig.	 &	-0.18	 &	-1.42	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	645	\\ \hline
35	 &	díszít	 &	embellish	 &	OV	 &	-1.49	 &	-12.3	 &	\textsc{covering}	 &	1634	\\ \hline
36	 &	diszkriminál	 &	discriminate	 &	VO	 &	0.93	 &	4.09	 &	\textsc{affect}	 &	120	\\ \hline
37	 &	dokumentál	 &	document	 &	no sig.	 &	-0.02	 &	-0.12	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	327	\\ \hline
38	 &	dönget	 &	\begin{tabular}[c]{@{}l@{}}pound on,\\ hit on\end{tabular}	 &	OV	 &	-0.65	 &	-3.86	 &	\textsc{affect}	 &	248	\\ \hline
39	 &	dörzsöl	 &	rub	 &	VO	 &	0.61	 &	4.1	 &	\textsc{affect}	 &	378	\\ \hline
40	 &	drágít	 &	\begin{tabular}[c]{@{}l@{}}make more\\ expensive\end{tabular}	 &	VO	 &	1.83	 &	6.52	 &	\textsc{change}	 &	123	\\ \hline
41	 &	dúdol	 &	hum	 &	no sig.	 &	0.15	 &	0.68	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	108	\\ \hline
42	 &	éget	 &	burn	 &	no sig.	 &	0.23	 &	1.75	 &	\textsc{change}	 &	548	\\ \hline
43	 &	egyenget	 &	smooth	 &	no sig.	 &	0.08	 &	0.52	 &	\textsc{change}	 &	263	\\ \hline
44	 &	egységesít	 &	unify	 &	VO	 &	1.18	 &	6.43	 &	\textsc{change}	 &	242	\\ \hline
45	 &	egyszerűsít	 &	simplify	 &	VO	 &	1.38	 &	8.68	 &	\textsc{change}	 &	423	\\ \hline
46	 &	ékesít	 &	decorate	 &	OV	 &	-1.08	 &	-5	 &	\textsc{covering}	 &	146	\\ \hline
47	 &	éltet	 &	\begin{tabular}[c]{@{}l@{}}keep alive,\\ sustain\end{tabular}	 &	no sig.	 &	0.23	 &	1.74	 &	\textsc{affect}	 &	649	\\ \hline
48	 &	elemez	 &	analyze	 &	no sig.	 &	-0.03	 &	-0.28	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1137	\\ \hline
49	 &	\begin{tabular}[c]{@{}l@{}}elemez/\\ elemezik\end{tabular}	 &	analyze	 &	no sig.	 &	0.04	 &	0.37	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1384	\\ \hline
50	 &	élénkít	 &	vitalize	 &	VO	 &	1.16	 &	6.1	 &	\textsc{change}	 &	214	\\ \hline
51	 &	ellenez	 &	oppose	 &	VO	 &	1.59	 &	13.22	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1794	\\ \hline
52	 &	ellenőriz	 &	check, verify	 &	VO	 &	0.37	 &	3.34	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	2988	\\ \hline
53	 &	\begin{tabular}[c]{@{}l@{}}ellensúlyoz/\\ ellensúlyozik\end{tabular}	 &	counterbalance	 &	no sig.	 &	0.05	 &	0.42	 &	\textsc{covering}	 &	709	\\ \hline
54	 &	élvez/élvezik	 &	enjoy	 &	VO	 &	0.8	 &	7.49	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	6224	\\ \hline
55	 &	emelget	 &	lift	 &	VO	 &	0.73	 &	4.07	 &	\textsc{affect}	 &	212	\\ \hline
56	 &	enyhít	 &	ease	 &	VO	 &	1	 &	8.51	 &	\textsc{change}	 &	1531	\\ \hline
57	 &	érdemel	 &	deserve	 &	OV	 &	-1.43	 &	-11.39	 &	\textsc{ownership}	 &	1254	\\ \hline
58	 &	eredményez	 &	result in	 &	OV	 &	-2.75	 &	-18.11	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	1416	\\ \hline
59	 &	\begin{tabular}[c]{@{}l@{}}eredményez/\\ eredményezik\end{tabular}	 &	result in	 &	OV	 &	-2.13	 &	-18.64	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	4176	\\ \hline
60	 &	érint	 &	touch (on)	 &	OV	 &	-0.81	 &	-7.8	 &	\textsc{affect}	 &	17011	\\ \hline
61	 &	érlel	 &	ripen	 &	no sig.	 &	-0.19	 &	-0.93	 &	\textsc{change}	 &	126	\\ \hline
62	 &	erőltet	 &	force	 &	VO	 &	0.86	 &	6.44	 &	\textsc{affect}	 &	674	\\ \hline
63	 &	erősít	 &	strengthen	 &	no sig.	 &	0.03	 &	0.27	 &	\textsc{change}	 &	5690	\\ \hline
64	 &	\begin{tabular}[c]{@{}l@{}}értelmez/\\ értelmezik\end{tabular}	 &	\begin{tabular}[c]{@{}l@{}}interpret,\\ make sense of\end{tabular}	 &	VO	 &	0.45	 &	3.93	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1831	\\ \hline
65	 &	érvénytelenít	 &	void	 &	VO	 &	0.78	 &	5.4	 &	\textsc{change}	 &	460	\\ \hline
66	 &	érzékel	 &	perceive	 &	no sig.	 &	0.19	 &	1.66	 &	\textsc{perception}	 &	1836	\\ \hline
67	 &	érzékeltet	 &	make perceive	 &	no sig.	 &	0.07	 &	0.51	 &	?	 &	631	\\ \hline
68	 &	fájlal	 &	\begin{tabular}[c]{@{}l@{}}feel/express\\ pain\end{tabular}	 &	no sig.	 &	-0.17	 &	-0.97	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	218	\\ \hline
69	 &	fal	 &	devour	 &	VO	 &	1.44	 &	7.69	 &	\textsc{ingestion}	 &	262	\\ \hline
70	 &	favorizál	 &	favor	 &	OV	 &	-1.42	 &	-6.07	 &	\textsc{preference}	 &	144	\\ \hline
71	 &	fed	 &	cover	 &	OV	 &	-0.42	 &	-3.58	 &	\textsc{covering}	 &	1404	\\ \hline
72	 &	fejleszt	 &	develop	 &	no sig.	 &	0.08	 &	0.74	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	2691	\\ \hline
73	 &	fékez/fékezik	 &	put a halt to, break	 &	VO	 &	0.93	 &	6.26	 &	\textsc{affect}	 &	425	\\ \hline
74	 &	félt	 &	\begin{tabular}[c]{@{}l@{}}worry about,\\ be protective of\end{tabular}	 &	VO	 &	0.67	 &	5.73	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1377	\\ \hline
75	 &	fémjelez	 &	mark (a metal)	 &	OV	 &	-0.42	 &	-2.2	 &	\textsc{change}	 &	166	\\ \hline
76	 &	fen	 &	hone	 &	VO	 &	1.89	 &	6.22	 &	\textsc{change}	 &	107	\\ \hline
77	 &	fenyeget	 &	threaten	 &	OV	 &	-0.59	 &	-5.44	 &	\textsc{affect}	 &	3373	\\ \hline
78	 &	\begin{tabular}[c]{@{}l@{}}fényképez/\\ fényképezik\end{tabular}	 &	photograph	 &	no sig.	 &	-0.24	 &	-1.52	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	286	\\ \hline
79	 &	fertőtlenít	 &	disinfect	 &	no sig.	 &	0.23	 &	1.24	 &	\textsc{change}	 &	178	\\ \hline
80	 &	feszeget	 &	\begin{tabular}[c]{@{}l@{}}literal: stretch;\\ figurative: discuss,\\ stretch the\\boundaries of\end{tabular}	 &	OV	 &	-0.87	 &	-6.47	 &	?	 &	640	\\ \hline
81	 &	finomít	 &	refine	 &	VO	 &	0.68	 &	3.51	 &	\textsc{change}	 &	164	\\ \hline
82	 &	firtat	 &	dwell on	 &	OV	 &	-1.19	 &	-7.61	 &	\textsc{activity}	 &	403	\\ \hline
83	 &	foglalkoztat	 &	employ, occupy	 &	OV	 &	-1.16	 &	-10.06	 &	\textsc{activity}	 &	2046	\\ \hline
84	 &	fogyaszt	 &	consume	 &	OV	 &	-0.91	 &	-8.23	 &	\textsc{ingestion}	 &	3163	\\ \hline
85	 &	fojtogat	 &	choke (iterative)	 &	no sig.	 &	0.15	 &	0.78	 &	\textsc{affect}	 &	143	\\ \hline
86	 &	fokoz/fokozik	 &	intensify, elevate	 &	VO	 &	0.61	 &	5.62	 &	\textsc{change}	 &	3262	\\ \hline
87	 &	fontolgat	 &	\begin{tabular}[c]{@{}l@{}}ponder upon\\ a decision\end{tabular}	 &	OV	 &	-0.79	 &	-6.25	 &	\textsc{preference}	 &	835	\\ \hline
88	 &	forradalmasít	 &	revolutionize	 &	VO	 &	1.65	 &	7.88	 &	\textsc{change}	 &	223	\\ \hline
89	 &	fosztogat	 &	loot (iterative)	 &	no sig.	 &	-0.04	 &	-0.21	 &	\textsc{affect}	 &	147	\\ \hline
90	 &	frissít	 &	refresh	 &	VO	 &	0.73	 &	5.55	 &	\textsc{change}	 &	654	\\ \hline
91	 &	fürkész	 &	scan, examine	 &	no sig.	 &	-0.28	 &	-1.6	 &	\textsc{perception}	 &	211	\\ \hline
92	 &	fűt	 &	heat	 &	no sig.	 &	0.04	 &	0.28	 &	\textsc{change}	 &	333	\\ \hline
93	 &	garantál	 &	guarantee	 &	VO	 &	0.48	 &	4.19	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1618	\\ \hline
94	 &	gátol	 &	obstruct	 &	VO	 &	0.83	 &	7.25	 &	\textsc{affect}	 &	1761	\\ \hline
95	 &	generál	 &	generate	 &	OV	 &	-1.33	 &	-9.54	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	679	\\ \hline
96	 &	gerjeszt	 &	induce	 &	OV	 &	-0.7	 &	-5.18	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	571	\\ \hline
97	 &	\begin{tabular}[c]{@{}l@{}}gondoz/\\ gondozik\end{tabular}	 &	care for	 &	no sig.	 &	-0.06	 &	-0.49	 &	\textsc{affect}	 &	714	\\ \hline
98	 &	gúnyol	 &	mock	 &	no sig.	 &	0.19	 &	0.88	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	119	\\ \hline
99	 &	gyaláz	 &	revile	 &	no sig.	 &	0.17	 &	1	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	210	\\ \hline
100	 &	gyarapít	 &	breed	 &	OV	 &	-0.41	 &	-3.21	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	717	\\ \hline
101	 &	gyászol	 &	mourn	 &	OV	 &	-0.55	 &	-3.7	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	367	\\ \hline
102	 &	gyengít	 &	weaken	 &	VO	 &	0.82	 &	6.63	 &	\textsc{change}	 &	1024	\\ \hline
103	 &	gyógyít	 &	heal	 &	no sig.	 &	0.15	 &	1.12	 &	\textsc{change}	 &	500	\\ \hline
104	 &	gyorsít	 &	accelerate	 &	VO	 &	1.3	 &	9.22	 &	\textsc{change}	 &	639	\\ \hline
105	 &	gyűlöl	 &	hate	 &	VO	 &	1.74	 &	13.58	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1330	\\ \hline
106	 &	habzsol	 &	devour	 &	VO	 &	2.52	 &	6.98	 &	\textsc{ingestion}	 &	121	\\ \hline
107	 &	hajszol	 &	rush	 &	VO	 &	0.48	 &	2.75	 &	\textsc{affect}	 &	212	\\ \hline
108	 &	halogat	 &	\begin{tabular}[c]{@{}l@{}}postpone\\ (iterative)\end{tabular}	 &	VO	 &	1.46	 &	8.8	 &	\textsc{change}	 &	383	\\ \hline
109	 &	hall	 &	hear	 &	OV	 &	-1.52	 &	-7.23	 &	\textsc{perception}	 &	201	\\ \hline
110	 &	hallat	 &	\begin{tabular}[c]{@{}l@{}}make heard\end{tabular}	 &	no sig.	 &	-0.13	 &	-1.01	 &	?	 &	568	\\ \hline
111	 &	hall/hallik	 &	hear	 &	OV	 &	-0.56	 &	-5.35	 &	\textsc{perception}	 &	17557	\\ \hline
112	 &	hamisít	 &	\begin{tabular}[c]{@{}l@{}}make a fake\\ version of\end{tabular}	 &	no sig.	 &	-0.07	 &	-0.48	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	334	\\ \hline
113	 &	hanyagol	 &	neglect	 &	VO	 &	0.4	 &	2.17	 &	\textsc{affect}	 &	177	\\ \hline
114	 &	hatástalanít	 &	deactivate	 &	no sig.	 &	0.32	 &	1.97	 &	\textsc{change}	 &	268	\\ \hline
115	 &	hátráltat	 &	hinder	 &	VO	 &	0.63	 &	5.16	 &	\textsc{affect}	 &	1016	\\ \hline
116	 &	helyesel	 &	approve	 &	VO	 &	1.23	 &	8.78	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	635	\\ \hline
117	 &	helytelenít	 &	disapprove of	 &	VO	 &	1.31	 &	6.5	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	198	\\ \hline
118	 &	hívogat	 &	call	 &	VO	 &	0.56	 &	2.51	 &	\textsc{affect}	 &	110	\\ \hline
119	 &	hiányol	 &	miss	 &	VO	 &	0.37	 &	3.07	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1024	\\ \hline
120	 &	hibáztat	 &	blame	 &	OV	 &	-1.31	 &	-9.01	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	561	\\ \hline
121	 &	hitelesít	 &	\begin{tabular}[c]{@{}l@{}}authenticate,\\ validate\end{tabular}	 &	VO	 &	0.49	 &	3.38	 &	\textsc{change}	 &	420	\\ \hline
122	 &	hullat	 &	shed	 &	no sig.	 &	0.23	 &	1.03	 &	\textsc{affect}	 &	106	\\ \hline
123	 &	húzogat	 &	pull (iterative)	 &	VO	 &	0.51	 &	2.38	 &	\textsc{affect}	 &	120	\\ \hline
124	 &	idéz	 &	cite, remind	 &	no sig.	 &	0.14	 &	1.35	 &	?	 &	7603	\\ \hline
125	 &	igazgat	 &	direct, manage	 &	OV	 &	-0.53	 &	-3.69	 &	?	 &	414	\\ \hline
126	 &	igazol	 &	certify	 &	no sig.	 &	-0.05	 &	-0.47	 &	\textsc{change}	 &	3402	\\ \hline
127	 &	igényel	 &	demand, need	 &	OV	 &	-1.18	 &	-11.15	 &	\textsc{ownership}	 &	8727	\\ \hline
128	 &	ihlet	 &	inspire	 &	OV	 &	-0.86	 &	-6.64	 &	\textsc{change}	 &	785	\\ \hline
129	 &	illet	 &	belong to	 &	OV	 &	-3.27	 &	-28.62	 &	\textsc{ownership}	 &	11303	\\ \hline
130	 &	illusztrál	 &	illustrate	 &	OV	 &	-0.52	 &	-3.75	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	481	\\ \hline
131	 &	imád	 &	worship, adore	 &	VO	 &	1.74	 &	15.72	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	4491	\\ \hline
132	 &	imitál	 &	imitate	 &	no sig.	 &	0.2	 &	1.08	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	171	\\ \hline
133	 &	indukál	 &	induce	 &	OV	 &	-1.43	 &	-6.27	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	155	\\ \hline
134	 &	ingat	 &	destabilize	 &	VO	 &	0.66	 &	4.67	 &	\textsc{change}	 &	478	\\ \hline
135	 &	ingerel	 &	irritate, nettle	 &	VO	 &	0.47	 &	2.46	 &	\textsc{change}	 &	166	\\ \hline
136	 &	inspirál	 &	inspire	 &	OV	 &	-0.57	 &	-4.12	 &	\textsc{change}	 &	499	\\ \hline
137	 &	irigyel	 &	envy	 &	VO	 &	1.16	 &	8.32	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	613	\\ \hline
138	 &	irritál	 &	irritate	 &	VO	 &	0.79	 &	4.77	 &	\textsc{change}	 &	273	\\ \hline
139	 &	ismer	 &	know (someone)	 &	VO	 &	0.78	 &	7.51	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	26934	\\ \hline
140	 &	iszik	 &	drink	 &	VO	 &	0.23	 &	2.11	 &	\textsc{ingestion}	 &	3329	\\ \hline
141	 &	ízesít	 &	spice	 &	no sig.	 &	-0.09	 &	-0.58	 &	\textsc{change}	 &	316	\\ \hline
142	 &	ízlel	 &	taste	 &	VO	 &	1.28	 &	5.6	 &	\textsc{ingestion}	 &	142	\\ \hline
143	 &	javít	 &	repair	 &	VO	 &	0.79	 &	7.28	 &	\textsc{change}	 &	4061	\\ \hline
144	 &	jelent	 &	mean	 &	OV	 &	-1.43	 &	-13.67	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	20776	\\ \hline
145	 &	jelez	 &	indicate	 &	OV	 &	-0.82	 &	-7.68	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	5713	\\ \hline
146	 &	\begin{tabular}[c]{@{}l@{}}jelképez/\\ jelképezik\end{tabular}	 &	symbolize	 &	OV	 &	-1.39	 &	-11.21	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	1303	\\ \hline
147	 &	jellemez	 &	characterize	 &	OV	 &	-0.43	 &	-4.01	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	4390	\\ \hline
148	 &	\begin{tabular}[c]{@{}l@{}}jellemez/\\ jellemezik\end{tabular}	 &	describe	 &	no sig.	 &	-0.17	 &	-1.51	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	2738	\\ \hline
149	 &	kárhoztat	 &	condemn	 &	no sig.	 &	0.29	 &	1.6	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	180	\\ \hline
150	 &	károsít	 &	impair	 &	VO	 &	0.77	 &	6.29	 &	\textsc{change}	 &	1022	\\ \hline
151	 &	kártalanít	 &	indemnify	 &	VO	 &	0.85	 &	3.98	 &	\textsc{change}	 &	134	\\ \hline
152	 &	kedvel	 &	like	 &	no sig.	 &	-0.16	 &	-1.46	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	4989	\\ \hline
153	 &	kémlel	 &	spy on, observe	 &	no sig.	 &	-0.12	 &	-0.66	 &	\textsc{perception}	 &	187	\\ \hline
154	 &	képez/képezik	 &	form, constitute	 &	OV	 &	-1.49	 &	-13.87	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	6752	\\ \hline
155	 &	képvisel	 &	represent	 &	OV	 &	-1.26	 &	-11.92	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	8610	\\ \hline
156	 &	keres	 &	search for	 &	no sig.	 &	-0.11	 &	-1.05	 &	\textsc{activity}	 &	22114	\\ \hline
157	 &	\begin{tabular}[c]{@{}l@{}}keresztez/\\ keresztezik\end{tabular}	 &	\begin{tabular}[c]{@{}l@{}}cross (someone's\\ way)\end{tabular}	 &	VO	 &	0.62	 &	4.29	 &	\textsc{affect}	 &	413	\\ \hline
158	 &	kerülget	 &	\begin{tabular}[c]{@{}l@{}}go around\\ (iterative)\end{tabular}	 &	VO	 &	0.56	 &	3.73	 &	\textsc{covering}	 &	373	\\ \hline
159	 &	késleltet	 &	delay	 &	VO	 &	0.75	 &	5.41	 &	\textsc{change}	 &	527	\\ \hline
160	 &	kevesell	 &	deem little	 &	VO	 &	1.52	 &	9.44	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	441	\\ \hline
161	 &	kifogásol	 &	expostulate	 &	no sig.	 &	-0.04	 &	-0.36	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1790	\\ \hline
162	 &	kímél	 &	spare	 &	no sig.	 &	0.14	 &	1.16	 &	\textsc{change}	 &	1134	\\ \hline
163	 &	kockáztat	 &	risk	 &	OV	 &	-0.56	 &	-4.31	 &	?	 &	667	\\ \hline
164	 &	kódol	 &	encode	 &	OV	 &	-1	 &	-5.04	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	178	\\ \hline
165	 &	kommentál	 &	comment on	 &	VO	 &	1.24	 &	10.77	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	2093	\\ \hline
166	 &	kontrollál	 &	control	 &	VO	 &	0.64	 &	3.38	 &	\textsc{affect}	 &	179	\\ \hline
167	 &	konzervál	 &	conserve	 &	VO	 &	0.75	 &	4.06	 &	\textsc{change}	 &	196	\\ \hline
168	 &	koordinál	 &	coordinate	 &	no sig.	 &	0.03	 &	0.2	 &	\textsc{affect}	 &	616	\\ \hline
169	 &	koptat	 &	wear down	 &	no sig.	 &	0.17	 &	1.02	 &	\textsc{change}	 &	221	\\ \hline
170	 &	\begin{tabular}[c]{@{}l@{}}korlátoz/\\ korlátozik\end{tabular}	 &	constrain, limit	 &	VO	 &	0.7	 &	6.46	 &	\textsc{affect}	 &	3468	\\ \hline
171	 &	\begin{tabular}[c]{@{}l@{}}koronáz/\\ koronázik\end{tabular}	 &	crown, coronate	 &	OV	 &	-1.5	 &	-9.06	 &	?	 &	396	\\ \hline
172	 &	korrigál	 &	correct	 &	VO	 &	0.67	 &	4.64	 &	\textsc{change}	 &	429	\\ \hline
173	 &	korszerűsít	 &	modernize	 &	VO	 &	0.8	 &	5.16	 &	\textsc{change}	 &	351	\\ \hline
174	 &	kortyol	 &	take sips of	 &	VO	 &	0.53	 &	2.72	 &	\textsc{ingestion}	 &	159	\\ \hline
175	 &	\begin{tabular}[c]{@{}l@{}}körvonalaz/\\ körvonalazik\end{tabular}	 &	outline	 &	no sig.	 &	0.04	 &	0.18	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	100	\\ \hline
176	 &	kóstál	 &	?	 &	OV	 &	-4.85	 &	-4.84	 &	?	 &	129	\\ \hline
177	 &	köszön	 &	thank	 &	VO	 &	2.07	 &	19.76	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	21747	\\ \hline
178	 &	követ	 &	follow	 &	OV	 &	-0.28	 &	-2.65	 &	\textsc{covering}	 &	12532	\\ \hline
179	 &	kritizál	 &	criticize	 &	VO	 &	0.4	 &	3.46	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1385	\\ \hline
180	 &	kutat	 &	research	 &	OV	 &	-0.57	 &	-4.86	 &	\textsc{activity}	 &	1441	\\ \hline
181	 &	lapátol	 &	shovel	 &	VO	 &	0.97	 &	4.24	 &	\textsc{change}	 &	120	\\ \hline
182	 &	lapozgat	 &	\begin{tabular}[c]{@{}l@{}}turn the pages of\\ (iterative)\end{tabular}	 &	no sig.	 &	-0.19	 &	-1.01	 &	\textsc{activity}	 &	172	\\ \hline
183	 &	lassít	 &	slow	 &	VO	 &	1.42	 &	11.04	 &	\textsc{change}	 &	1072	\\ \hline
184	 &	latolgat	 &	\begin{tabular}[c]{@{}l@{}}ponder upon\\ (a decision)\end{tabular}	 &	no sig.	 &	-0.34	 &	-1.91	 &	\textsc{preference}	 &	197	\\ \hline
185	 &	legitimál	 &	legitimate	 &	VO	 &	1.07	 &	4.89	 &	\textsc{change}	 &	141	\\ \hline
186	 &	les	 &	expect, watch for	 &	VO	 &	0.56	 &	4.53	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	913	\\ \hline
187	 &	likvidál	 &	liquidate	 &	VO	 &	0.6	 &	2.67	 &	\textsc{change}	 &	110	\\ \hline
188	 &	lóbál	 &	swing	 &	VO	 &	0.48	 &	2.22	 &	\textsc{affect}	 &	120	\\ \hline
189	 &	lobogtat	 &	\begin{tabular}[c]{@{}l@{}}wave some canvas\\ (e.g. a flag)\end{tabular}	 &	OV	 &	-0.42	 &	-2.28	 &	\textsc{affect}	 &	172	\\ \hline
190	 &	lógat	 &	hang	 &	VO	 &	1.03	 &	5.73	 &	\textsc{affect}	 &	236	\\ \hline
191	 &	magasztal	 &	extol	 &	no sig.	 &	0.27	 &	1.58	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	226	\\ \hline
192	 &	manipulál	 &	manipulate	 &	VO	 &	0.95	 &	6.28	 &	\textsc{change}	 &	405	\\ \hline
193	 &	markol	 &	grasp, hold onto	 &	no sig.	 &	0.2	 &	1.15	 &	\textsc{affect}	 &	198	\\ \hline
194	 &	másol	 &	copy	 &	no sig.	 &	-0.02	 &	-0.14	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	382	\\ \hline
195	 &	masszíroz	 &	massage	 &	no sig.	 &	0.1	 &	0.47	 &	\textsc{affect}	 &	124	\\ \hline
196	 &	mellőz	 &	ignore	 &	VO	 &	0.5	 &	3.85	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	663	\\ \hline
197	 &	méltányol	 &	appreciate	 &	VO	 &	0.71	 &	4.36	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	277	\\ \hline
198	 &	mélyít	 &	aggravate	 &	VO	 &	1.39	 &	7.33	 &	\textsc{change}	 &	246	\\ \hline
199	 &	menedzsel	 &	manage	 &	no sig.	 &	0.38	 &	1.9	 &	?	 &	145	\\ \hline
200	 &	méreget	 &	\begin{tabular}[c]{@{}l@{}}measure\\ (iterative)\end{tabular}	 &	VO	 &	1	 &	4.81	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	156	\\ \hline
201	 &	mereszt	 &	\begin{tabular}[c]{@{}l@{}}open (the eyes) wide\end{tabular}	 &	VO	 &	0.72	 &	3.69	 &	\textsc{change}	 &	165	\\ \hline
202	 &	\begin{tabular}[c]{@{}l@{}}mérgez/\\mérgezik\end{tabular}	 &	poison	 &	VO	 &	1.4	 &	7.06	 &	\textsc{change}	 &	218	\\ \hline
203	 &	mérlegel	 &	weigh	 &	VO	 &	0.47	 &	3.8	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	847	\\ \hline
204	 &	minimalizál	 &	minimize	 &	VO	 &	0.94	 &	4.73	 &	\textsc{change}	 &	171	\\ \hline
205	 &	moderál	 &	moderate	 &	VO	 &	1.5	 &	5.85	 &	\textsc{affect}	 &	121	\\ \hline
206	 &	modernizál	 &	modernize	 &	VO	 &	0.64	 &	3.65	 &	\textsc{change}	 &	220	\\ \hline
207	 &	molesztál	 &	molest	 &	VO	 &	0.54	 &	2.56	 &	\textsc{affect}	 &	130	\\ \hline
208	 &	mormol	 &	murmur	 &	OV	 &	-0.9	 &	-3.68	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	100	\\ \hline
209	 &	mos	 &	wash	 &	VO	 &	0.37	 &	2.97	 &	\textsc{affect}	 &	818	\\ \hline
210	 &	motivál	 &	motivate	 &	OV	 &	-0.28	 &	-2.15	 &	\textsc{change}	 &	639	\\ \hline
211	 &	mozgat	 &	make move	 &	no sig.	 &	0.13	 &	1.13	 &	\textsc{change}	 &	1140	\\ \hline
212	 &	mutogat	 &	point at (iterative)	 &	OV	 &	-0.4	 &	-2.85	 &	\textsc{covering}	 &	482	\\ \hline
213	 &	művel	 &	cultivate	 &	OV	 &	-0.74	 &	-5.86	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	848	\\ \hline
214	 &	nehezít	 &	make more difficult	 &	no sig.	 &	-0.03	 &	-0.24	 &	\textsc{change}	 &	2925	\\ \hline
215	 &	nélkülöz	 &	lack	 &	VO	 &	0.67	 &	5.45	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	970	\\ \hline
216	 &	nemz	 &	father, sire	 &	OV	 &	-0.79	 &	-3.62	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	125	\\ \hline
217	 &	nevel	 &	grow, cultivate	 &	OV	 &	-0.34	 &	-3.05	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	1961	\\ \hline
218	 &	nevesít	 &	name, label	 &	no sig.	 &	0.24	 &	1.25	 &	?	 &	161	\\ \hline
219	 &	nézeget	 &	look at	 &	VO	 &	0.45	 &	3.85	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1446	\\ \hline
220	 &	növeszt	 &	grow	 &	OV	 &	-0.88	 &	-4.74	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	204	\\ \hline
221	 &	nyal	 &	lick	 &	no sig.	 &	0.33	 &	1.93	 &	\textsc{affect}	 &	229	\\ \hline
222	 &	nyalogat	 &	lick	 &	no sig.	 &	-0.23	 &	-1.52	 &	\textsc{affect}	 &	308	\\ \hline
223	 &	nyitogat	 &	open (iterative)	 &	VO	 &	0.47	 &	2.18	 &	\textsc{affect}	 &	117	\\ \hline
224	 &	nyomogat	 &	press (iterative)	 &	OV	 &	-0.37	 &	-2.08	 &	\textsc{affect}	 &	205	\\ \hline
225	 &	nyomkod	 &	nyomkod	 &	VO	 &	1.18	 &	6.17	 &	\textsc{affect}	 &	213	\\ \hline
226	 &	nyugtalanít	 &	make concerned	 &	OV	 &	-0.71	 &	-3.75	 &	\textsc{change}	 &	179	\\ \hline
227	 &	nyújtogat	 &	stretch	 &	VO	 &	0.49	 &	2.15	 &	\textsc{change}	 &	105	\\ \hline
228	 &	okoz/okozik	 &	cause	 &	OV	 &	-0.72	 &	-6.91	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	22121	\\ \hline
229	 &	ölt	 &	stitch	 &	OV	 &	-2.22	 &	-12.74	 &	\textsc{affect}	 &	571	\\ \hline
230	 &	olvas	 &	read	 &	VO	 &	0.21	 &	2.03	 &	\textsc{ingestion}	 &	9886	\\ \hline
231	 &	olvasgat	 &	read	 &	VO	 &	0.39	 &	2.55	 &	\textsc{ingestion}	 &	336	\\ \hline
232	 &	öntöz	 &	irrigate	 &	no sig.	 &	-0.34	 &	-1.68	 &	\textsc{affect}	 &	137	\\ \hline
233	 &	őriz	 &	guard	 &	OV	 &	-0.25	 &	-2.29	 &	\textsc{covering}	 &	3985	\\ \hline
234	 &	orvosol	 &	solve, heal	 &	no sig.	 &	0.09	 &	0.71	 &	\textsc{change}	 &	650	\\ \hline
235	 &	összegez	 &	\begin{tabular}[c]{@{}l@{}}conclude,\\ summarize\end{tabular}	 &	no sig.	 &	0.16	 &	1.07	 &	?	 &	335	\\ \hline
236	 &	\begin{tabular}[c]{@{}l@{}}összegez/\\ összegezik\end{tabular}	 &	summarize	 &	VO	 &	1.1	 &	8.24	 &	\textsc{change}	 &	733	\\ \hline
237	 &	összesít	 &	summarize	 &	OV	 &	-0.42	 &	-2.63	 &	?	 &	280	\\ \hline
238	 &	\begin{tabular}[c]{@{}l@{}}osztályoz/\\ osztályozik\end{tabular}	 &	classify	 &	VO	 &	1.57	 &	8.73	 &	\textsc{affect}	 &	324	\\ \hline
239	 &	óv	 &	guard	 &	VO	 &	1.23	 &	8.96	 &	\textsc{covering}	 &	697	\\ \hline
240	 &	övez/övezik	 &	surround	 &	OV	 &	-0.65	 &	-5.42	 &	\textsc{covering}	 &	1144	\\ \hline
241	 &	pártol	 &	support	 &	no sig.	 &	0.25	 &	1.68	 &	\textsc{affect}	 &	345	\\ \hline
242	 &	\begin{tabular}[c]{@{}l@{}}példáz/\\ példázik\end{tabular}	 &	exemplify	 &	OV	 &	-0.41	 &	-2.78	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	378	\\ \hline
243	 &	penget	 &	pluck (strings)	 &	OV	 &	-0.52	 &	-2.57	 &	\textsc{affect}	 &	142	\\ \hline
244	 &	pénzel	 &	support via money	 &	no sig.	 &	0.1	 &	0.58	 &	\textsc{affect}	 &	198	\\ \hline
245	 &	pihentet	 &	make rest	 &	VO	 &	0.55	 &	2.86	 &	\textsc{affect}	 &	159	\\ \hline
246	 &	piszkál	 &	pick on	 &	no sig.	 &	0.17	 &	1.06	 &	\textsc{affect}	 &	256	\\ \hline
247	 &	pontosít	 &	specify	 &	VO	 &	0.93	 &	6.67	 &	\textsc{change}	 &	558	\\ \hline
248	 &	\begin{tabular}[l]{@{}l@{}}pontoz/\\pontozik\end{tabular}	 &	score	 &	no sig.	 &	0.24	 &	1.05	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	102	\\ \hline
249	 &	pótol	 &	replace	 &	VO	 &	0.45	 &	3.96	 &	\textsc{change}	 &	1792	\\ \hline
250	 &	preferál	 &	prefer	 &	OV	 &	-1.4	 &	-9.03	 &	\textsc{preference}	 &	466	\\ \hline
251	 &	privatizál	 &	privatize	 &	no sig.	 &	-0.05	 &	-0.31	 &	\textsc{change}	 &	230	\\ \hline
252	 &	próbálgat	 &	try on	 &	no sig.	 &	-0.15	 &	-0.94	 &	\textsc{activity}	 &	302	\\ \hline
253	 &	propagál	 &	propagate ?	 &	no sig.	 &	-0.28	 &	-1.31	 &	\textsc{affect}	 &	114	\\ \hline
254	 &	provokál	 &	provoke	 &	VO	 &	0.96	 &	5.93	 &	\textsc{affect}	 &	324	\\ \hline
255	 &	rág	 &	chew	 &	VO	 &	0.44	 &	3.27	 &	\textsc{affect}	 &	571	\\ \hline
256	 &	rágcsál	 &	nibble	 &	no sig.	 &	-0.39	 &	-1.85	 &	\textsc{affect}	 &	126	\\ \hline
257	 &	ráncol	 &	crease	 &	no sig.	 &	0.29	 &	1.7	 &	\textsc{change}	 &	213	\\ \hline
258	 &	rángat	 &	pull around	 &	VO	 &	0.59	 &	3.91	 &	\textsc{affect}	 &	369	\\ \hline
259	 &	ratifikál	 &	ratify	 &	VO	 &	1.31	 &	7.58	 &	\textsc{change}	 &	307	\\ \hline
260	 &	ráz	 &	shake	 &	VO	 &	0.3	 &	2.63	 &	\textsc{affect}	 &	1594	\\ \hline
261	 &	rehabilitál	 &	rehabilitate	 &	VO	 &	0.55	 &	2.52	 &	\textsc{change}	 &	115	\\ \hline
262	 &	rejteget	 &	hide	 &	no sig.	 &	-0.18	 &	-1.19	 &	\textsc{covering}	 &	321	\\ \hline
263	 &	\begin{tabular}[c]{@{}l@{}}rendszerez/\\ rendszerezik\end{tabular}	 &	organize	 &	VO	 &	0.65	 &	3.19	 &	\textsc{affect}	 &	143	\\ \hline
264	 &	reprezentál	 &	represent	 &	OV	 &	-0.34	 &	-2.28	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	349	\\ \hline
265	 &	\begin{tabular}[c]{@{}l@{}}részletez/\\ részletezik\end{tabular}	 &	detail	 &	VO	 &	0.32	 &	2.41	 &	\textsc{change}	 &	580	\\ \hline
266	 &	ritkít	 &	\begin{tabular}[c]{@{}l@{}}interspace,\\ make sparser\end{tabular}	 &	OV	 &	-1.01	 &	-5.23	 &	\textsc{change}	 &	191	\\ \hline
267	 &	rombol	 &	destroy	 &	VO	 &	0.6	 &	4.39	 &	\textsc{change}	 &	518	\\ \hline
268	 &	roncsol	 &	damage	 &	VO	 &	1.09	 &	4.82	 &	\textsc{change}	 &	131	\\ \hline
269	 &	ront	 &	spoil	 &	VO	 &	0.78	 &	7.04	 &	\textsc{change}	 &	2735	\\ \hline
270	 &	rugdos	 &	kick (iterative)	 &	no sig.	 &	0.12	 &	0.65	 &	\textsc{affect}	 &	164	\\ \hline
271	 &	rühell	 &	hate	 &	VO	 &	1.18	 &	4.8	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	111	\\ \hline
272	 &	semlegesít	 &	neutralize	 &	VO	 &	0.58	 &	3.56	 &	\textsc{change}	 &	278	\\ \hline
273	 &	serkent	 &	stimulate	 &	VO	 &	1.51	 &	10.18	 &	\textsc{change}	 &	591	\\ \hline
274	 &	sért	 &	offend	 &	VO	 &	0.5	 &	4.7	 &	\textsc{change}	 &	4902	\\ \hline
275	 &	sérteget	 &	\begin{tabular}[c]{@{}l@{}}hurt, offend\\ (iterative)\end{tabular}	 &	VO	 &	1.43	 &	5.53	 &	\textsc{affect}	 &	114	\\ \hline
276	 &	siettet	 &	urge	 &	VO	 &	1.26	 &	7.03	 &	\textsc{affect}	 &	271	\\ \hline
277	 &	simogat	 &	pet	 &	no sig.	 &	0.17	 &	1.33	 &	\textsc{affect}	 &	697	\\ \hline
278	 &	sirat	 &	mourn	 &	no sig.	 &	-0.14	 &	-1.01	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	422	\\ \hline
279	 &	skandál	 &	\begin{tabular}[l]{@{}l@{}}loudly, repeatedly\\say\end{tabular}	 &	OV	 &	-1.66	 &	-7.94	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	225	\\ \hline
280	 &	sokall	 &	deem too much	 &	VO	 &	1.17	 &	7.62	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	423	\\ \hline
281	 &	sokkol	 &	shock	 &	VO	 &	0.34	 &	2.39	 &	\textsc{change}	 &	444	\\ \hline
282	 &	stabilizál	 &	stabilize	 &	VO	 &	1.22	 &	8.23	 &	\textsc{change}	 &	503	\\ \hline
283	 &	stimulál	 &	stimulate	 &	VO	 &	0.79	 &	3.92	 &	\textsc{change}	 &	154	\\ \hline
284	 &	súlyosbít	 &	exasperate	 &	no sig.	 &	0.15	 &	1.23	 &	\textsc{change}	 &	844	\\ \hline
285	 &	sürget	 &	urge	 &	OV	 &	-0.55	 &	-4.98	 &	\textsc{affect}	 &	2563	\\ \hline
286	 &	súrol	 &	scour	 &	no sig.	 &	-0.2	 &	-1.44	 &	\textsc{affect}	 &	462	\\ \hline
287	 &	\begin{tabular}[c]{@{}l@{}}szabályoz/\\ szabályozik\end{tabular}	 &	regulate	 &	no sig.	 &	-0.17	 &	-1.62	 &	\textsc{change}	 &	3630	\\ \hline
288	 &	szabotál	 &	sabotage	 &	VO	 &	1.52	 &	6.02	 &	\textsc{change}	 &	128	\\ \hline
289	 &	szagol	 &	smell	 &	no sig.	 &	0.06	 &	0.29	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	138	\\ \hline
290	 &	számolgat	 &	enumerate	 &	no sig.	 &	0.35	 &	1.56	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	104	\\ \hline
291	 &	szankcionál	 &	sanction	 &	no sig.	 &	0.01	 &	0.07	 &	?	 &	163	\\ \hline
292	 &	szaporít	 &	breed	 &	VO	 &	0.46	 &	2.99	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	311	\\ \hline
293	 &	szaval	 &	recite	 &	OV	 &	-0.66	 &	-3.38	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	164	\\ \hline
294	 &	szavatol	 &	warrant	 &	VO	 &	0.54	 &	3.69	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	394	\\ \hline
295	 &	szeg	 &	nail, frame	 &	OV	 &	-0.52	 &	-3.22	 &	?	 &	281	\\ \hline
296	 &	\begin{tabular}[c]{@{}l@{}}szegélyez/\\ szegélyezik\end{tabular}	 &	frame	 &	OV	 &	-1.14	 &	-6.36	 &	\textsc{covering}	 &	252	\\ \hline
297	 &	szélesít	 &	broaden	 &	VO	 &	0.78	 &	4.21	 &	\textsc{change}	 &	197	\\ \hline
298	 &	szemléltet	 &	show, illustrate	 &	OV	 &	-1.08	 &	-7.41	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	490	\\ \hline
299	 &	\begin{tabular}[c]{@{}l@{}}szennyez/\\ szennyezik\end{tabular}	 &	contaminate	 &	VO	 &	1.27	 &	8.08	 &	\textsc{change}	 &	418	\\ \hline
300	 &	szentesít	 &	approve	 &	VO	 &	1.07	 &	6.46	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	310	\\ \hline
301	 &	szerkeszt	 &	edit	 &	OV	 &	-1.01	 &	-8.77	 &	?	 &	1902	\\ \hline
302	 &	szív	 &	suck	 &	VO	 &	0.41	 &	2.14	 &	\textsc{affect}	 &	158	\\ \hline
303	 &	szid	 &	scold	 &	VO	 &	0.47	 &	3.79	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	864	\\ \hline
304	 &	\begin{tabular}[c]{@{}l@{}}szidalmaz/\\ szidalmazik\end{tabular}	 &	scold	 &	VO	 &	0.51	 &	2.51	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	141	\\ \hline
305	 &	szigorít	 &	tighten, toughen	 &	VO	 &	2.02	 &	13.06	 &	\textsc{change}	 &	725	\\ \hline
306	 &	szimbolizál	 &	symbolize	 &	OV	 &	-1.6	 &	-11.29	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	759	\\ \hline
307	 &	szimulál	 &	simulate	 &	no sig.	 &	-0.35	 &	-1.64	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	114	\\ \hline
308	 &	színesít	 &	color	 &	VO	 &	0.36	 &	2.7	 &	\textsc{change}	 &	574	\\ \hline
309	 &	színez/színezik	 &	color	 &	no sig.	 &	-0.02	 &	-0.12	 &	\textsc{change}	 &	182	\\ \hline
310	 &	szív	 &	suck	 &	VO	 &	0.52	 &	4.21	 &	\textsc{affect}	 &	904	\\ \hline
311	 &	szolgál	 &	serve	 &	OV	 &	-1.51	 &	-14.31	 &	?	 &	10865	\\ \hline
312	 &	szoptat	 &	breast-feed	 &	no sig.	 &	0.1	 &	0.44	 &	\textsc{affect}	 &	103	\\ \hline
313	 &	\begin{tabular}[c]{@{}l@{}}szorgalmaz/\\ szorgalmazik\end{tabular}	 &	urge, hasten	 &	OV	 &	-0.77	 &	-6.93	 &	\textsc{affect}	 &	2417	\\ \hline
314	 &	szorongat	 &	squeeze	 &	no sig.	 &	-0.15	 &	-1.07	 &	\textsc{affect}	 &	443	\\ \hline
315	 &	szponzorál	 &	sponsor	 &	no sig.	 &	-0.28	 &	-1.39	 &	\textsc{affect}	 &	137	\\ \hline
316	 &	szűkít	 &	make narrower	 &	VO	 &	1.14	 &	8.24	 &	\textsc{change}	 &	639	\\ \hline
317	 &	szül	 &	give birth to	 &	OV	 &	-0.69	 &	-6.03	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	1841	\\ \hline
318	 &	tágít	 &	broaden	 &	VO	 &	1.03	 &	5.8	 &	\textsc{change}	 &	244	\\ \hline
319	 &	taglal	 &	elaborate on	 &	OV	 &	-1.08	 &	-7.01	 &	\textsc{activity}	 &	402	\\ \hline
320	 &	takar	 &	cover	 &	OV	 &	-1.58	 &	-12.96	 &	\textsc{covering}	 &	1640	\\ \hline
321	 &	támogat	 &	support, donate	 &	VO	 &	0.56	 &	5.39	 &	\textsc{affect}	 &	24224	\\ \hline
322	 &	\begin{tabular}[c]{@{}l@{}}tanulmányoz/\\ tanulmányozik\end{tabular}	 &	study	 &	VO	 &	0.23	 &	2.04	 &	\textsc{ingestion}	 &	2199	\\ \hline
323	 &	tanúsít	 &	be a sign of	 &	OV	 &	-1.56	 &	-11.8	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	1003	\\ \hline
324	 &	táplál	 &	feed (sustain)	 &	no sig.	 &	-0.08	 &	-0.65	 &	\textsc{affect}	 &	1177	\\ \hline
325	 &	tapogat	 &	\begin{tabular}[c]{@{}l@{}}feel with the\\ fingers, touch\end{tabular}	 &	no sig.	 &	-0.31	 &	-1.94	 &	\textsc{affect}	 &	283	\\ \hline
326	 &	\begin{tabular}[c]{@{}l@{}}tárcsáz/\\ tárcsázik\end{tabular}	 &	dial	 &	VO	 &	0.66	 &	3.07	 &	\textsc{affect}	 &	126	\\ \hline
327	 &	tarkít	 &	fleck	 &	no sig.	 &	-0.23	 &	-1.43	 &	\textsc{change}	 &	260	\\ \hline
328	 &	tartalmaz	 &	contain	 &	OV	 &	-1.26	 &	-11.94	 &	\textsc{covering}	 &	10791	\\ \hline
329	 &	\begin{tabular}[c]{@{}l@{}}tartalmaz/\\ tartalmazik\end{tabular}	 &	contain	 &	OV	 &	-0.57	 &	-5.48	 &	\textsc{covering}	 &	17560	\\ \hline
330	 &	tehermentesít	 &	disencumber	 &	VO	 &	0.97	 &	4.68	 &	\textsc{change}	 &	156	\\ \hline
331	 &	teljesít	 &	fulfil	 &	VO	 &	0.49	 &	4.65	 &	\textsc{change}	 &	6881	\\ \hline
332	 &	terhel	 &	burden	 &	OV	 &	-0.66	 &	-5.97	 &	\textsc{affect}	 &	2586	\\ \hline
333	 &	termel	 &	produce	 &	OV	 &	-1.07	 &	-9.25	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	1852	\\ \hline
334	 &	tervezget	 &	plan	 &	no sig.	 &	-0.26	 &	-1.45	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	195	\\ \hline
335	 &	tetéz	 &	intensify, pile on	 &	OV	 &	-0.65	 &	-4.2	 &	\textsc{change}	 &	340	\\ \hline
336	 &	\begin{tabular}[c]{@{}l@{}}tisztáz/\\tisztázik\end{tabular}	 &	clear up	 &	VO	 &	0.99	 &	8.3	 &	\textsc{change}	 &	1380	\\ \hline
337	 &	tisztít	 &	clean	 &	VO	 &	0.64	 &	4.43	 &	\textsc{affect}	 &	439	\\ \hline
338	 &	tökéletesít	 &	improve	 &	VO	 &	0.65	 &	3.89	 &	\textsc{change}	 &	259	\\ \hline
339	 &	tologat	 &	pull	 &	VO	 &	0.46	 &	2.27	 &	\textsc{affect}	 &	137	\\ \hline
340	 &	tolerál	 &	tolerate	 &	VO	 &	0.92	 &	5.29	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	252	\\ \hline
341	 &	tömörít	 &	compactify	 &	OV	 &	-1.59	 &	-8.95	 &	\textsc{change}	 &	341	\\ \hline
342	 &	tompít	 &	make blunter	 &	VO	 &	0.69	 &	4.12	 &	\textsc{change}	 &	260	\\ \hline
343	 &	tördel	 &	break at	 &	no sig.	 &	0.25	 &	1.33	 &	\textsc{affect}	 &	160	\\ \hline
344	 &	törölget	 &	wipe (iterative)	 &	no sig.	 &	-0.12	 &	-0.63	 &	\textsc{affect}	 &	174	\\ \hline
345	 &	torzít	 &	distort	 &	VO	 &	1.03	 &	6.48	 &	\textsc{change}	 &	350	\\ \hline
346	 &	\begin{tabular}[c]{@{}l@{}}tükröz/\\tükrözik\end{tabular}	 &	mirror	 &	OV	 &	-0.55	 &	-5.13	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	4684	\\ \hline
347	 &	túr	 &	dig	 &	VO	 &	0.88	 &	3.97	 &	\textsc{affect}	 &	126	\\ \hline
348	 &	tűr	 &	tolerate	 &	VO	 &	1.34	 &	11.01	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1431	\\ \hline
349	 &	üdvözöl	 &	greet	 &	VO	 &	1.89	 &	16.44	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	3267	\\ \hline
350	 &	üldöz	 &	chase	 &	no sig.	 &	0.17	 &	1.32	 &	\textsc{affect}	 &	688	\\ \hline
351	 &	un	 &	be bored by	 &	VO	 &	1.97	 &	14.55	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	1205	\\ \hline
352	 &	ural	 &	dominate	 &	VO	 &	0.43	 &	3.79	 &	\textsc{affect}	 &	2044	\\ \hline
353	 &	utál	 &	hate	 &	VO	 &	1.67	 &	14.16	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	2240	\\ \hline
354	 &	utánoz	 &	imitate	 &	no sig.	 &	-0.11	 &	-0.82	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	594	\\ \hline
355	 &	üzemeltet	 &	operate	 &	OV	 &	-1.21	 &	-10.02	 &	\textsc{activity}	 &	1379	\\ \hline
356	 &	vakar	 &	scratch, scrape	 &	VO	 &	0.45	 &	2.58	 &	\textsc{affect}	 &	206	\\ \hline
357	 &	választ	 &	choose	 &	OV	 &	-0.89	 &	-8.49	 &	\textsc{preference}	 &	14679	\\ \hline
358	 &	váltogat	 &	\begin{tabular}[c]{@{}l@{}}switch back\\ and forth\end{tabular}	 &	VO	 &	1.23	 &	6.77	 &	\textsc{change}	 &	256	\\ \hline
359	 &	variál	 &	\begin{tabular}[c]{@{}l@{}}change back\\ and forth\end{tabular}	 &	OV	 &	-0.75	 &	-3.29	 &	\textsc{change}	 &	112	\\ \hline
360	 &	vázol	 &	sketch	 &	VO	 &	0.95	 &	6.66	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	503	\\ \hline
361	 &	véd	 &	protect	 &	no sig.	 &	0.05	 &	0.46	 &	\textsc{covering}	 &	4816	\\ \hline
362	 &	vedel	 &	drink (a lot of)	 &	OV	 &	-1	 &	-4.17	 &	\textsc{ingestion}	 &	108	\\ \hline
363	 &	\begin{tabular}[c]{@{}l@{}}védelmez/\\ védelmezik\end{tabular}	 &	protect	 &	no sig.	 &	0.17	 &	1.18	 &	\textsc{covering}	 &	434	\\ \hline
364	 &	\begin{tabular}[c]{@{}l@{}}véleményez/\\ véleményezik\end{tabular}	 &	opine on	 &	VO	 &	0.76	 &	5.24	 &	\begin{tabular}[c]{@{}c@{}}\textsc{evaluation/}\\\textsc{experience}\end{tabular}	 &	442	\\ \hline
365	 &	vereget	 &	hit at	 &	no sig.	 &	0.21	 &	0.96	 &	\textsc{affect}	 &	103	\\ \hline
366	 &	veszélyeztet	 &	endanger	 &	no sig.	 &	-0.03	 &	-0.28	 &	\textsc{change}	 &	6502	\\ \hline
367	 &	vét	 &	\begin{tabular}[c]{@{}l@{}}make a mistake,\\ offend\end{tabular}	 &	OV	 &	-2.57	 &	-9.23	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	226	\\ \hline
368	 &	vezérel	 &	guide, motivate	 &	OV	 &	-0.32	 &	-2.55	 &	\textsc{affect}	 &	771	\\ \hline
369	 &	villant	 &	flash	 &	OV	 &	-1.04	 &	-4.81	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	142	\\ \hline
370	 &	visel	 &	wear, bear	 &	OV	 &	-0.84	 &	-8	 &	\textsc{covering}	 &	11483	\\ \hline
371	 &	\begin{tabular}[c]{@{}l@{}}visszhangoz/\\ visszhangozik/\\ visszhangzik\end{tabular}	 &	echo	 &	OV	 &	-0.78	 &	-3.56	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	124	\\ \hline
372	 &	viszonoz	 &	requite	 &	VO	 &	1.5	 &	10.09	 &	?	 &	581	\\ \hline
373	 &	vizionál	 &	envision	 &	OV	 &	-1.95	 &	-6.83	 &	\begin{tabular}[c]{@{}c@{}}\textsc{creation/}\\\textsc{representation}\end{tabular}	 &	129	\\ \hline
374	 &	vizsgál	 &	examine	 &	OV	 &	-0.64	 &	-6.11	 &	\textsc{perception}	 &	10098	\\ \hline
375	 &	vonogat	 &	pull	 &	OV	 &	-0.53	 &	-3.36	 &	\textsc{affect}	 &	297	\\ \hline
376	 &	zabál	 &	gobble	 &	VO	 &	0.56	 &	2.96	 &	\textsc{ingestion}	 &	173	\\ \hline
377	 &	zaklat	 &	molest	 &	VO	 &	0.56	 &	3.86	 &	\textsc{affect}	 &	400	\\ \hline
378	 &	zárol	 &	lock (down)	 &	VO	 &	0.6	 &	4.36	 &	\textsc{change}	 &	509	\\ \hline
379	 &	zavar	 &	disturb	 &	no sig.	 &	0.16	 &	1.51	 &	\textsc{change}	 &	2922	\\ \hline
380	 &	zsákmányol	 &	prey, obtain	 &	OV	 &	-2.8	 &	-10.85	 &	\textsc{affect}	&	330	\\ \hline  
\end{longtable}
